Localized Conformal Prediction for Image Classification with Vision-Language Models

Conformal predictions have attracted significant attention in the field of uncertainty quantification, mainly because of their strong marginal coverage guarantees. Full conditional guarantee is not an attainable goal, a well known fact in conformal predictions literature. As a result, several approaches have tried to approximate this behavior by adapting the conformal sets of test-time samples according to their similarity to calibration examples. Although the latter has gained traction and shown impressive performances for regression problems, its application to image classification remains under-explored. We conduct an extensive benchmarking on natural image classification tasks with vision-language models (VLMs), using our open source implementation of a recent localized conformal prediction algorithm. We show that straightforward usage of the cosine similarity between test-time and calibration visual features, an intuitive choice for VLMs, is not sufficient to improve over the non-local baselines. In response, we propose a simple non-linear transformation of the cosine similarities, which conserves marginal coverage guarantees and achieves statistically significant mean set sizes reduction. Code is available at https://github.com/cfuchs2023/lcp-vlm/.

==> tables/rn50_cvg.tex <==
% Adjust white spaces of mid and top rules
\aboverulesep = 0.1mm %default 0.605mm
\belowrulesep = 0.1mm %default 0.984mm


\setlength\dashlinedash{0.2pt}
                        \setlength\dashlinegap{1.5pt}
                        \setlength\arrayrulewidth{0.3pt}
                        \renewcommand{\arraystretch}{1.}
                        \begin{table*}[]
                            \caption{RN50 CovGap MCCC
        }
    \label{tab:results}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccccccc}
          \toprule

 & \rotatebox[origin=c]{45}{UCF101} & \rotatebox[origin=c]{45}{dtd} & \rotatebox[origin=c]{45}{OxfordPets} & \rotatebox[origin=c]{45}{eurosat} & \rotatebox[origin=c]{45}{StanfordCars} & \rotatebox[origin=c]{45}{Flower102} & \rotatebox[origin=c]{45}{fgvc_aircraft} & \rotatebox[origin=c]{45}{sun397} & \rotatebox[origin=c]{45}{Food101} 

\\ \midrule

\textbf{Zero-Shot} & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ & $\text{0.000}$ \\ \midrule

 TOPK  &\fontsize{11}{11}{\underline{\textcolor{black}{0.12}}}/\text{\textcolor{black}{0.02}}&\text{\textcolor{black}{0.12}}/\text{\textcolor{black}{0.03}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.07}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.48}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.81}}}&\text{\textcolor{black}{0.10}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.14}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.00}}}&\text{\textcolor{black}{0.11}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.00}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.05}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.70}}}

\\ \cmidrule(l){2-10}

 LOCAL - COSINE - TOPK &\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.12}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.04}}}&\text{\textcolor{black}{0.07}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.48}}}&\text{\textcolor{black}{0.11}}/\text{\textcolor{black}{0.68}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.10}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}&\text{\textcolor{black}{0.15}}/\text{\textcolor{black}{0.00}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\text{\textcolor{black}{0.00}}&\text{\textcolor{black}{0.08}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.05}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.70}}}

\\ \cmidrule(l){2-10}

 \cellcolor{pink} LOCAL - TOPK &\cellcolor{pink} \text{\textcolor{black}{0.12}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.02}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.14}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.06}}}/\cellcolor{pink} \text{\textcolor{black}{0.48}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.76}}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.10}}}/\cellcolor{pink} \text{\textcolor{black}{0.08}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.14}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.01}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.10}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.00}}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}/\cellcolor{pink} \text{\textcolor{black}{0.03}}&\cellcolor{pink} \text{\textcolor{black}{0.05}}/\cellcolor{pink} \text{\textcolor{black}{0.68}}

\\ \cmidrule(l){2-10}

 LAC  &\text{\textcolor{black}{0.12}}/\text{\textcolor{black}{0.02}}&\text{\textcolor{black}{0.12}}/\text{\textcolor{black}{0.09}}&\text{\textcolor{black}{0.07}}/\text{\textcolor{black}{0.35}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.09}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.70}}}&\text{\textcolor{black}{0.10}}/\text{\textcolor{black}{0.08}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.14}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.00}}}&\text{\textcolor{black}{0.11}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.01}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}/\text{\textcolor{black}{0.02}}&\text{\textcolor{black}{0.05}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.66}}}

\\ \cmidrule(l){2-10}

 LOCAL - COSINE - LAC &\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.13}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.07}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.39}}}&\text{\textcolor{black}{0.09}}/\text{\textcolor{black}{0.68}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.10}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.09}}}&\text{\textcolor{black}{0.15}}/\text{\textcolor{black}{0.00}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\text{\textcolor{black}{0.01}}&\text{\textcolor{black}{0.08}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.05}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.70}}}

\\ \cmidrule(l){2-10}

 \cellcolor{pink} LOCAL - LAC &\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.12}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.03}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.19}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.07}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.42}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.07}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.75}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.10}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.14}}}/\cellcolor{pink} \text{\textcolor{black}{0.00}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.01}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.03}}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.05}}}/\cellcolor{pink} \text{\textcolor{black}{0.66}}

\\ \cmidrule(l){2-10}

 APS  &\text{\textcolor{black}{0.11}}/\text{\textcolor{black}{0.08}}&\text{\textcolor{black}{0.12}}/\text{\textcolor{black}{0.10}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.07}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.90}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.06}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.83}}}&\text{\textcolor{black}{0.09}}/\text{\textcolor{black}{0.19}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.14}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.00}}}&\text{\textcolor{black}{0.11}}/\text{\textcolor{black}{0.00}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.09}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.05}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.81}}}

\\ \cmidrule(l){2-10}

 LOCAL - COSINE - APS &\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.13}}}&\text{\textcolor{black}{0.07}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.90}}}&\text{\textcolor{black}{0.06}}/\text{\textcolor{black}{0.81}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.09}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.21}}}&\text{\textcolor{black}{0.14}}/\text{\textcolor{black}{0.00}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.01}}}&\text{\textcolor{black}{0.08}}/\text{\textcolor{black}{0.09}}&\text{\textcolor{black}{0.06}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.83}}}

\\ \cmidrule(l){2-10}

 \cellcolor{pink} LOCAL - APS &\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.18}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.07}}}/\cellcolor{pink} \text{\textcolor{black}{0.90}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.06}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.83}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.09}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.19}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.14}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.01}}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.00}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.09}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.05}}}/\cellcolor{pink} \text{\textcolor{black}{0.81}}

\\ \cmidrule(l){2-10}

 RAPS  &\fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.04}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.12}}}/\text{\textcolor{black}{0.05}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.07}}}/\text{\textcolor{black}{0.81}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.72}}}&\text{\textcolor{black}{0.09}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.12}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.15}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.00}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.00}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.08}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.03}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.05}}}/\text{\textcolor{black}{0.75}}

\\ \cmidrule(l){2-10}

 LOCAL - COSINE - RAPS &\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.04}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.12}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.06}}}&\text{\textcolor{black}{0.08}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.81}}}&\fontsize{11}{11}{\underline{\textcolor{black}{0.09}}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.71}}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.09}}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.12}}}&\text{\textcolor{black}{0.15}}/\text{\textcolor{black}{0.00}}&\fontsize{11}{11}{\textbf{\textcolor{black}{0.11}}}/\text{\textcolor{black}{0.00}}&\text{\textcolor{black}{0.08}}/\fontsize{11}{11}{\underline{\textcolor{black}{0.03}}}&\text{\textcolor{black}{0.05}}/\fontsize{11}{11}{\textbf{\textcolor{black}{0.76}}}

\\ \cmidrule(l){2-10}

 \cellcolor{pink} LOCAL - RAPS &\cellcolor{pink} \text{\textcolor{black}{0.11}}/\cellcolor{pink} \text{\textcolor{black}{0.04}}&\cellcolor{pink} \text{\textcolor{black}{0.12}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.06}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.07}}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.81}}}&\cellcolor{pink} \text{\textcolor{black}{0.12}}/\cellcolor{pink} \text{\textcolor{black}{0.52}}&\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.09}}}/\cellcolor{pink} \text{\textcolor{black}{0.11}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.15}}}/\cellcolor{pink} \text{\textcolor{black}{0.00}}&\cellcolor{pink} \text{\textcolor{black}{0.12}}/\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.00}}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.08}}}/\cellcolor{pink} \text{\textcolor{black}{0.03}}&\cellcolor{pink} \fontsize{11}{11}{\textbf{\textcolor{black}{0.05}}}/\cellcolor{pink} \fontsize{11}{11}{\underline{\textcolor{black}{0.75}}}

\\ \cmidrule(l){2-10}

\end{tabular}}
\end{table*}
